Data Augmentation for Dementia Detection in Spoken Language

Dementia is a growing problem as our society ages, and detection methods are often invasive and expensive. Recent deep-learning techniques can offer a faster diagnosis and have shown promising results. However, they require large amounts of labelled data which is not easily available for the task of dementia detection. One effective solution to sparse data problems is data augmentation, though the exact methods need to be selected carefully. To date, there has been no empirical study of data augmentation on Alzheimer's disease (AD) datasets for NLP and speech processing. In this work, we investigate data augmentation techniques for the task of AD detection and perform an empirical evaluation of the different approaches on two kinds of models for both the text and audio domains. We use a transformer-based model for both domains, and SVM and Random Forest models for the text and audio domains, respectively. We generate additional samples using traditional as well as deep learning based methods and show that data augmentation improves performance for both the text- and audio-based models and that such results are comparable to state-of-the-art results on the popular ADReSS set, with carefully crafted architectures and features.

==> 07_Future_Work_old.tex <==
\section{Limitations, Challenges \& Future Directions}
\label{sec:future}

\subsubsection{Cross-corpus analysis \& regression task}
A clear limitation of our work is the focus on a small dataset for dementia detection, a subset of relatively small set itself. However, the the small size of this dataset makes perfect to experiment with data augmentation. We are also able to directly compare our work to the ones previously submitted for the challenge as we use the same test set. However, it would be valuable to investigate the impact of the various data augmentation techniques across different dementia datasets. In this work we report our experiments on the task of classification only. Some of the selected transformations we described here did not give us good results for the regression task, possibly because the connection between feature distribution and the given score is very fragile. However this is an interesting direction to explore further.

\subsubsection{Beyond common augmentations} 
The scope of this paper is to evaluate common and well known techniques for data augmentations. We did not, however, explore more fine-tuned methods that would exploit domain knowledge and feature engineering. With such approaches, one needs to be careful not to introduce features that would be disruptive to the classification task and thus would require deeper understanding of discriminatory features for each class. However, it has been previously shown that dyslfuency features and syntactic information are important features. Future work would craft augmentation techniques making use of this information.

\subsubsection{Explainable data augmentations}
It has become more and more desirable to be able to explain why different approaches work and how reliable the predictions are, even more so in the domain of healthcare. Explainable models could help us better understand the impact the different data augmentation have and why some are more successful than other.    
\subsubsection{Style transfer}
As generative models become better and better at synthesizing speech they could be really helpful at augmenting datasets that will be close to real data. Approaches that investigate one-shot or zero-shot style transfer on both text and speech would eventually become powerful techniques to solve the limited dataset issues omnipresent in fields related to healthcare. 

\subsubsection{Data-level fusion}
Many of the data augmentations in text presented in our work do not have an obvious overlap with the speech ones and thus were evaluated separately. As a result our fusion strategies had to be separate as well and are done in a late-fusion manner. However, an interesting direction to explore are multi-modal data augmentation techniques that would translate to both text and audio on data level. The text augmentations could be coupled with a TTS model that would transfer the linguistic information back to the speech domain. This would also include online data augmentation more similar to what is being done in the field of computer vision, as opposed to the offline data augmentations presented in this paper.

\subsubsection{Practical considerations}
When picking augmentation methods it is important to take into consideration not only the impact on the model performance but also the additional overhead to run these methods and optimize them. These include running time and the number of parameters to optimize. Recent literature explore automatic data augmentation search done on the fly on the task of interest but they have yet to be evaluated on different tasks and domains.


==> 08_Related_Work.tex <==
\section{Related Work in Data Augmentation For Dementia Detection}
\label{sec:rel_work}

In this work we focused on the main data augmentation strategies for text and audio domains. Papers by~\cite{liu2021detecting} and~\cite{ye2021development} implement general techniques that we explored such as masking and speed change. However, there exist several other techniques and variations that we did not explore in this paper and that were applied to Dementia classification. 
In~\cite{guo2021crossing}, the authors take advantage of another existing text dataset for dementia to train a model with on a larger corpus and help with overfitting. 
We do not have access to another dataset that provide both text and audio samples. Nevertheless, it is a future direction to explore, perhaps even with non-parallel sets. 
An indirect form of augmentation is to split the words and waveforms into phonemes and subwords as done by author et al.~\cite{}. Doing so they increase their sample sizes while decrease the vocabulary. Features on the phonemes level also highlight dysfluencies that patients with dementia often produce when they speak and improve the model discriminatory power.









